Spin Excitation Spectrum of La$_{1-x}A_x$MnO$_3$

As an effective model to describe perovskite-type manganates (La,$A$)MnO$_3$, the double-exchange model on a cubic lattice is investigated. Spin excitation spectrum of the model in the ground state is studied using the spin wave approximation. Spin wave dispersion relation observed in the inelastic neutron scattering experiment of La$_{0.7}$Pb$_{0.3}$MnO$_3$ is reproduced. Effective values for the electron bandwidth as well as Hund's coupling is estimated from the data.

==> dxsfig.tex <==
%auto-ignore
\newpage
\section*{Figure Captions}

\begin{figure}
\hfil\epsfile{file=SelfEnergy.eps,scale=\figscaleB}\hfil
\caption{Spin wave self energy in the lowest order of the $1/S$ expansion. 
Green's functions for electrons
and spin wave are given by bold and wavy curves, respectively.
Vertices for $xy$ and $z$ couplings are represented by circles and 
a square, respectively.}
\label{FigSWPi}
\end{figure}

\begin{figure}
\hfil\epsfile{file=Disp.eps,scale=\figscaleA}\hfil
\caption{Spin wave dispersion relation at $x=0.3$.
Curves are for $\JH/t=\infty$, $24$, $12$ and $6$ from top to bottom.}
\label{FigSpinDisp}
\end{figure}


%
\begin{figure}
\hfil\epsfile{file=Fit.Disp.eps,scale=\figscaleA}\hfil
\caption{Spin wave dispersion relation of \LaPbMnO (squares)
from ref.~\citen{Perring95x}.
Curves are calculated by fitting data at $\JH/t=12$ (dotted curve)
 and $\JH/t = \infty$ (solid curve).}
\label{FigNeutron}
\end{figure}
%

\begin{figure}
\hfil\epsfile{file=Esw.D.eps,scale=\figscaleA}\hfil
\caption{Magnon bandwidth $\Esw$ (solid curve)
 and the spin stiffness $D_{\rm s}$ (dashed line) at $x=0.3$.}
\label{FigEswD}
\end{figure}


